Dynamic Operational Planning in Warfare: A Stochastic Game Approach to Military Campaigns

We study a two-player discounted zero-sum stochastic game model for dynamic operational planning in military campaigns. At each stage, the players manage multiple commanders who order military actions on objectives that have an open line of control. When a battle over the control of an objective occurs, its stochastic outcome depends on the actions and the enabling support provided by the control of other objectives. Each player aims to maximize the cumulative number of objectives they control, weighted by their criticality. To solve this large-scale stochastic game, we derive properties of its Markov perfect equilibria by leveraging the logistics and military operational command and control structure. We show the consequential isotonicity of the optimal value function with respect to the partially ordered state space, which in turn leads to a significant reduction of the state and action spaces. We also accelerate Shapley's value iteration algorithm by eliminating dominated actions and investigating pure equilibria of the matrix game solved at each iteration. We demonstrate the computational value of our equilibrium results on a case study that reflects representative operational-level military campaigns with geopolitical implications. Our analysis reveals a complex interplay between the game's parameters and dynamics in equilibrium, resulting in new military insights for campaign analysts.

==> Sec_1_Intro1.tex <==
%!TEX root = NRL Manuscript.tex
\section{Introduction}

\md{Similarly, I invite you to read Onkar's and Lacy's most recent introduction sections. It will give you an idea on how to organize this section. Typically, it goes as follows:

- Motivation (challenges + opportunities)

- Short summary of gaps in the literature (short, because you will expand in the lit review section)

- Main research question

- Detailed description of contributions.


It's important, when you write a section/some paragraphs, to make a mental map of the information you are providing. Right now, the first thing you mention is 0-sum stochastic game for operational-level military analysis. Then you talk about levels of warfare. But zero-sum game will not be mentioned for a very long time (suggesting it was not needed in that first sentence).}

The zero-sum stochastic game presents an opportunity for operational-level military analysis. There are three levels of warfare: strategic, operational and tactical, where the operational level links the tactical employment of forces to national strategic objectives \citepalias{jp3-0}. At the operational level, Joint Force Commanders employ military forces to deter adversaries and support multinational partners at the geopolitical scale \citepalias{jp3-0}. Campaign analysis, a method which applies models and techniques to answer questions about operational-level military operations, yields geopolitical insights and recommendations for senior decision makers \citep{teco21}. Campaign analysis applies scenarios --- plausible military settings that focus the military force --- to answer questions about military operations, e.g., \cite{shla16, maza19}. Campaign analysis is the most aggregated level of military modeling and simulation (M\&S) lying above mission, engagement, and engineering-level models in order of decreasing aggregation \citep{wade20}. Because it represents the operational level, campaign analysis influences wide-reaching decisions made at the strategic level. Historic military campaigns such as Waterloo, Stalingrad, and Normandy all helped determine the outcome of major geopolitical conflicts. \md{I don't fully understand the point you are making here. The description is good, but after reading it, my question is: so what? That's because I cannot see the main thread and the link between the different pieces of information you are providing.}

Campaign analysis, through computer simulation or wargaming, helps assess geopolitical, strategic, and operational possibilities. These tools often link strategic-level decisions, such as investment in assets or activities, to operational-level impacts, e.g., \cite{muel16, flan19} \md{Do we care much about strategic in this paper?}. Furthermore, operational warfare is the realization of many tactical-level decisions. Accordingly, we define \md{We don't usually introduce any definition in an introduction. The purpose of the introduction is to motivate and describe the main research question, and summarize the contributions} the military campaign as an operational-level representation of strategic investment in manning, training, and equipping as demonstrated through sequential tactical-level battles. With this definition in mind, we contend that the framework demonstrated in this paper links the three levels of warfare.

There are various models the military uses for campaign analysis. Staff members often rely on roundtable format, “political-military” (POL-MIL) games. These seminar style games are a great step towards identifying key elements of global competition. For operational problems, the military often relies on tabletop wargames to simulate combat operations. These games take days to assess military options against one adversary course of action and they are sensitive to player priorities, dominating personalities, and wargame rules. Simulation is another approach that produces results faster than a wargame. However, the campaign simulations often take months to build and can be  data intensive. Most importantly, all of these approaches take time and can only evaluate one scenario (e.g., force mix or starting conditions) at a time. \md{This previous paragraph is a bit in-between, in my opinion. In the literature review, you will want to explain in details what is usually done for campaign analysis (provide citations, and describe the limitations). Here, we only want a quick summary of the current approaches/limitations to introduce the gaps and motivate the research question you will work on.

Next paragraph, you will then directly state the research question. And only after, as part of the contributions, you will explain that you introduce a zero-sum stochastic game, etc.}

We model the military campaign as a zero-sum stochastic game. Although our framework may not provide the detail of a wargame or simulation \md{No need to downplay your model here. Focus on the positive side (and if there are limitations, you can frame them as a ``tradeoff'')}, it aims to yield quick, first-order assessments \md{This is about the impact/benefits of the model. I would keep this as the last set of contributions (you end the contributions by explaining who would benefit from your work (and how))}. This responsiveness allows the decision maker (DM) to evaluate a wide range of input scenarios. We seek to provide timely insights and first-order recommendations for strategic and operational decision making. 

%\jm{Gap in existing research}
While the zero-sum stochastic game (often called a Markov game or competitive game) is a well established framework starting in the 1950s \citep{rag91, shap53} \md{Now you are going back to some quick lit review. This needs some reorganization}, the construct has not been extensively applied to military campaign analysis. To our knowledge, no existing research has framed an operational-level campaign as zero-sum game using our approach \md{To be merged with some of the limitations mentioned above. This statement can also be changed a bit. Instead of saying no campaign has been framed as a zero-sum game, you can instead say that there is no decision model for campaign analysis that considers the dynamic and stochastic aspect of military campaigns. (something like this). After the research question, you can then say you introduce the zero-sum game. It's better than saying (there is no zero-sum game, so we introduce a zero-sum game).}. Military analysts and operational-level planners have much to gain from this construct \citep{wash14} \md{Now this is again regarding who would benefit from it. (to be reoganized)}. Solving the game yields the Markov perfect equilibrium (MPE) policy and value, which provides insights to operational-level planners and campaign outcomes to strategic-level force developers. 

%\jm{Main research question} 
At the outset we ask, can we model a military campaign as a stochastic game while maintaining sufficient resolution and computational efficiency for a responsive decision support system (DSS)? \md{Main research question will have to be adjusted. Something less technical that does not mention the stochastic game. (check Onkar's, Bastián's, or Lacy's) } We summarize this paper's contribution \md{That will need to be expanded. Please check my other papers to have a good idea on the amount of details to include}: 

%In this paper we build a military campaign with a special structure to reduce our state and action space. We solve or approximate the MPE policies and value through accelerated value iteration (AVI) and a heuristic we develop. 

\begin{itemize}
    \item We apply the structure of military operations to express the state and action space.
    \item We develop AVI and a heuristic which allows us to find or approximate the campaign's MPE.
    \item We demonstrate the efficacy of the zero-sum stochastic game for the military campaign analysis community.
\end{itemize}

We trust that this framework provides a strong foundation for a military DSS.


\md{Most papers finish the introduction section with a paragraph outlining the paper (please check my other papers for examples)}

==> Sec_1_Intro_MathieuNotes.tex <==
%!TEX root = NRL Manuscript.tex
\section{Introduction}

\subsection{Motivation}

%%%% 1st para: Warfare in general %%%%
An era of great power competition poses a challenge for military leadership \citepalias{hqda21}. The military must posture to deter great power competition from becoming armed conflict \citepalias{hqda21}, yet the military must still plan for potential armed conflict scenarios. Operational-level warfare is intrinsically complex and dynamic, where one commander's domain or region is intertwined or co-dependent with another domain or region. Commanders must work together to achieve the best result against an adversary who also fights across domains. 

%%%% 2nd para. Campaign Analysis Introduction as part of opnl planning %%%%
Operational-level warfare links the tactical employment of forces to national strategic objectives \citepalias{jp3-0}. At this level, Joint Force Commanders lead component commanders (e.g., air, land, and maritime) across domains to fight conflicts. Campaign analysis models these military operations, to yield geopolitical insights and recommendations for senior decision makers \citep{teco21, muel16, shla16, flan19, maza19}. Strategists, planners, and analysts alike employ \emph{campaign analysis} to produce operations plans for these uncertain contingencies and provide insights to military leadership. \cite{teco21} submit that campaign analysis manages ``uncertainty to answer questions about military operations". Indeed, the product of campaign analysis is often a concept of operations (CONOP) which links these intertwined domains to produce a unified strategy.

%%%% 3rd para. Challenges related to campaign analysis %%%%
% Uncertainty, Dynamic, Strategic

%%%% 4th para. Current state of lit. and gaps %%%%

%%%TO DO: What source talks about campaign analysis

Combat simulations and wargaming are two campaign analysis tools which are often used individually or in tandem to study combat \citep{turn22}.


\subsection{Motivation with notes}

\md{After going through 1.1, I feel there are a few repetitions, and some reorganization of the paragraphs is needed. My main issue is that campaign analysis, tactical/operational/strategic appear multiple times throughout.

One option is to have:
1st paragraph about warfare in general (without necessarily mentioning campaign analysis)

2nd paragraph that introduces campaign analysis as an important part of operational planning. And you can describe it there.

3rd paragraph about challenges related to campaign analysis

4th paragraph about brief current state of the literature and gaps. Meaning, currently, tools to perform campaign analysis include wargaming and simulation. However, here is the gap. Finish with main research question}

This prompts our research question: \emph{How may we responsively model dynamic military operations to yield quick-turn assessments, operational plans, and insights for senior leadership}?

An era of great power competition poses a challenge for military leadership \citepalias{hqda21}. The military must posture to deter great power competition from becoming armed conflict \citepalias{hqda21}, yet the military must still plan for potential armed conflict scenarios. Strategists, planners, and analysts alike employ \textit{campaign analysis} to plan for these uncertain contingencies and provide strategic and operational-level insights for military leadership. \md{You are already emphasizing strategic insights, although we barely address this in the paper.} 

%Compounded by the uncertainty of developing unpredictable scenarios, campaign analysis is inherently sequential and uncertain. This dynamic nature of the military campaign makes it inherently challenging to model. 

Operational-level warfare links the tactical employment of forces to national strategic objectives \citepalias{jp3-0}. At this level, Joint Force Commanders employ military forces to deter \md{In the first paragraph, I liked that you said: the first goal is to deter, but they also must plan for armed conflict. Here, you are back to only deterring. However, I don't think that's what we do. We don't mention deterrence in the main part of the paper.} adversaries and support multinational partners at the geopolitical scale \citepalias{jp3-0}. Campaign analysis models these military operations, to yield geopolitical insights and recommendations for senior decision makers \citep{teco21}. Campaign analysis links strategic-level decisions, such as investment in assets or activities, to operational-level impacts \md{I don't love this definition, as we barely do this linking. Can you adjust it to be closer to what we achieve in this paper?}, e.g., \cite{muel16, shla16,flan19, maza19}. Historical campaigns such as Waterloo, Stalingrad, and Normandy demonstrate that geopolitical outcomes and military campaigns are inseparable \md{I don't understand how this sentence ties with the previous one.}. 

%One campaign analysis scenario --- a plausible military setting that focuses the military force --- answers questions about military operations, e.g., \cite{shla16, maza19}. 

While campaign analysis bridges the gap between military operations and strategic decisions \md{Repetition, and I would hope to have a different emphasis for campaign analysis}, the domain comes with challenges. First, campaign outcomes are inherently uncertain due to the nature of warfare \md{Citation}. Second, a military campaign is not one discrete event, rather it may be envisioned as a sequence of military events (e.g., battles), where one outcome determines the next possible events. For instance during World War II, a successful allied D-Day invasion eventually led to Operation Market Garden, where U.S. and U.K. setbacks resulted in Russian forces reaching Berlin first \citep{hist19}. The uncertainty and dynamic, sequential aspects of military campaigns provide challenges and opportunities for our research. \md{Again a repetition and is not adding much. I would not mention ``out research'' yet. This is still part of the motivation (separate from us). As part of challenges, I would say the whole list is: uncertainty (you covered), dynamic (you partially covered: a dynamic problem in challenging in that future uncertain outcomes must be accounted for to optimize the present decision), and strategic (you didn't cover: You make a decision against another agent who is simultaneously making decisions)}

Some primary analytic tools for campaign analysis include wargaming and simulation. These tools are ideal for detailed analysis, operational planning, and assessing a single strategic decision. Yet, senior leadership often seeks campaign assessments for a range of decisions \md{The past two sentences are here to motivate this paper as a strategic decision paper, which it is not. Given that in the title we have operational planning, we have to show the value of this paper for operational decisions.}. However, each wargame or simulation can take days to months to execute. Current primary methods cannot quickly evaluate many strategic decisions.\md{I hope you see that this is not the main focus of the paper. This paragraph indeed serves as pointing out the gap in the literature. As such, each sentence needs one main citation (even if you cite it again in Section 2). If we recap the main limitations. Simulations are ideal for detailed dynamic analysis, but I would assume fail to account for the game-theoretic nature of the interactions. Is wargaming really ideal for detailed analysis? Or does it provide empirical analysis of game-theoretic interactions, but with decisions that hardly account for the complex uncertainty and dynamicity of the campaign? You can also have a sentence to explain that wargaming and simulation can take days to months to execute, and cannot be used as tools to quickly evaluate many strategic decisions (this is perfectly fine, as we address some of this).} This prompts our research question: \textit{How may we responsively model a military campaign to yield quick-turn assessments and insights for senior leadership}? \md{I like the second half of the question. The first half is too broad in my opinion. How to efficiently design optimal dynamic operational plans in warfare? You can have a second question: How to generate quick-turn assessments and military insights for senior leadership? (although I'm not sure we need a full second question for it). If you want to merge them: How to design optimal dynamic military operational plans and yield quick-turn assessments [and insight] for senior leadership?}

%Current tools, such as wargaming and computer simulation, take days to evaluate one scenario. Because strategic-level and operational-level decision makers (DMs) often require an assessment quickly, a more responsive campaign analysis tool is required. Furthermore, the opportunity exists for a first-order, aggregated campaign model to quickly screen a large amount of campaign starting states to yield candidate solutions worth of more detailed modeling through wargaming or simulation. This leads to our research question: \textit{How may we responsively model a military campaign to yield quick-turn assessments and insights for military decision makers}?

% FOR LIT REVIEW: Campaign analysis is the most aggregated level of military modeling and simulation (M\&S) lying above mission, engagement, and engineering-level models in order of decreasing aggregation \citep{wade20}. Because it represents the operational level, campaign analysis influences wide-reaching decisions made at the strategic level. Historic military campaigns such as Waterloo, Stalingrad, and Normandy all helped determine the outcome of major geopolitical conflicts.

%Today, in a world of great power competition, military leadership must make pivotal decisions to prepare for potential future armed conflict scenarios. 

%Strategic investment in technology, assets, and activities is inextricably linked with operational-level employment. Yet, it is challenging to quickly assess a strategic portfolio’s impact at the operational level. Current methods to explore the investment space are time intensive: to evaluate one portfolio a separate wargame or simulation must be run.

\subsection{Contributions}

To address the research question, we propose a novel two-person discounted zero-sum stochastic game model for dynamic operational planning in military campaigns, building upon the static game model of \cite{haywood54}. The features of the model account for key military features such as the coordination of multiple commanders, the need for established supply lines, and the stochasticity of battle outcomes that depend on the control of nearby objectives.

By leveraging the logistics and military operational
command and control structure we derive properties satisfied by the Markov perfect equilibria of the game. Under practically motivated assumptions, we show the nontrivial isotonicity of the optimal value function with respect to the partially ordered state space under (Theorem \ref{thm:isotone}). This main result, along with game-theoretic arguments, permit us to determine the set of achievable states as well as properties of policy profiles in equilibrium (Proposition \ref{prop:reduce}). This leads to a significant reduction of the state and action spaces, which in turn enables the use of Shapley's value iteration algorithm to solve this large-scale game.

In the special case of a campaign with one commander, we further show that the matrix game solved at most states within the value iteration algorithm admits weakly dominated strategies, and even admits a pure equilibrium when the commander manages a single axis of objectives
(Proposition \ref{prop:reduction}). These structural results lead us to design an accelerated value iteration algorithm (Algorithms \ref{alg:AZS}-\ref{alg:AVI}) that searches for pure equilibria or eliminates weakly dominated actions before solving
the matrix game using linear programming.


We then design a representative case study, built upon a fictional geopolitical scenario. We analyze and compare the players' mixed strategies at different states in equilibrium, and highlight a complex behavior that depends on  the criticalities of the objectives, the probabilistic
interdepedencies between objectives, and the dynamics of the game. We also show that strategic investment decisions must be carefully timed, as they have varied impacts on the optimal value of the game at different initial states. Finally, our equilibrium results permit us to solve the stochastic game for all considered military campaigns, using our accelerated value iteration algorithm that achieves a 72\% runtime reduction in comparison with the classical value iteration algorithm. Our analysis leads to novel operational insights that can be exploited by military leadership.


% our equilibrium


% Finally, our numerical analysis
% demonstrated the value of our equilibrium results in permitting us to efficiently solve the game
% with our accelerated value iteration algorithm for characteristic campaign instances that can be
% exploited by military decision makers.




The remainder of this article is organized as follows: Section \ref{sec:lit} reviews the existing literature \ul{on military applications of the stochastic game} \md{I don't like this. I believe it should be more broadly about military campaign analysis [and potentially also on military/defense game theory]. But I haven't read your lit review yet, so I can't finalize this yet.}. We formulate the stochastic game in Section \ref{sec:Pb}. We then derive our equilibrium results and present our accelerated value iteration algorithm in Section \ref{sec:approaches}. In Section \ref{sec:case_study}, we present our computational results and military insights from our case study. Section \ref{sec:conclusion} provides concluding remarks and avenues for future research. Finally, the mathematical proofs of our results are derived in Appendix \ref{app:deriv}.

% Section 6 lays out the concluding remarks and provides avenues for future research. Finally, the electronic companion (EC) contains mathematical proofs, detailed solution algorithms, and additional computational results.



% illustrates the application of our stochastic game modeling framework to a case study and 



% and presents the computational results and insights from a representative military campaigns



% the application of our stochastic game modeling framework and solution to a case study



% Section \ref{sec:case_study} illustrates the application of our technique to a case study. Furthermore we illustrate the tractability and accuracy of our solution approaches. Finally, Section \ref{sec:conclusion} provides a brief summary of our findings and direction for future research. 


 % which in turn lead to the applicability of Shapley’s value iteration



% lead to a significant reduction of the state and action spaces 


\subsection{\md{Old version of Contributions}}


To complement wargaming and simulation's role in campaign analysis we propose a third technique: the stochastic game. The ability to quickly evaluate campaigns allows us to responsively assess the risk of strategic decisions. The end-to-end approach we outline in the following portions delineates a novel methodology for campaign analysis. Specifically, we focus on the discounted, two-player, zero-sum stochastic game which avails nicely to military armed conflict \citep{wash14}. 

%Our campaign representation reflects sequential battles for military objectives. A battle may occur for these objectives depending on the stochastic flow of the campaign. The aggregation of our model allows the model to evaluate a wide range of input scenarios, thereby providing timely insights and first-order recommendations for strategic and operational decision making. 

%Our case study seeks to illustrate the approach and its pertinence to military analysis. We model the military campaign as a zero-sum stochastic game. Our model aggregates the major components of a military campaign into military objectives. 

%Formulation
The curse of dimensionality is a well-known challenge for stochastic games, so it is important to maintain a manageable state and action space. Accordingly, we exploit military supply lines and command structure to reflect military operations and create the state and action space for our stochastic game. The stochastic game output is the Markov perfect equilibrium (MPE). The MPE yields two pertinent outputs for decision makers: the strategy that both players should take from every possible campaign situation and the campaign risk measured as the total discounted expected loss.

%Approaches
We develop two solution approaches to find or approximate the MPE. First we modify Shapley's classic value iteration algorithm \citep{shap53} to converge to an $\epsilon$-MPE solution. We adapt the classical algorithm by first searching for a saddle point and, if necessary, removing dominated strategies. This accelerated value iteration (AVI) approach relies on solving matrix games to update the value until convergence. Our next solution approach also uses recursion and attempts to reduce the size of the matrix game using the commander's focused heuristic. Solving smaller matrix games allows us to complete iterations faster and arrive at an approximation faster. The output from this approximation may be used as a value warm start for AVI.

%Case Study
We tie our work together by demonstrating an end-to-end process of building the campaign model inputs, solving the model, and analyzing the outputs. We first create the campaign by translating military objectives, command structure, and logistics chains to the stochastic game formulation. Then we develop transition probabilities between the states by developing attacking and reinforcing probabilities for the players. Using our states, actions, and transition probabilities we find the MPE for the campaign stochastic game using both solution approaches. We conclude by comparing the two solution approaches.

%Contributions
We summarize our contributions accordingly:

\begin{itemize}
    \item We apply military command and logistics structure to develop the state and action space.
    \item We develop AVI and the CFH which finds or approximates the campaign's MPE.
    \item We demonstrate the efficacy of the zero-sum stochastic game for the campaign and the tractability of our solution approaches.
\end{itemize}

\md{I have not really used that paragraph. I don't like the focus on strategic decisions. But I think some of it is good. Feel free to merge with what I have.}Our target beneficiary is the military analytic community. With application of our methodology, we contend that analysts can deliver faster results to senior decision makers. Our model may assess many strategic decisions, before a more thorough review through wargaming and simulation. We believe the approach we outline in the following portions delineates a novel, responsive methodology for campaign analysis. 

The remainder of this paper is organized in five sections. Section \ref{sec:lit} reviews the existing literature on military applications of the stochastic game. We formulate the stochastic game in Section \ref{sec:Pb}. Section \ref{sec:approaches} lays out our two solution approaches. Section \ref{sec:case_study} illustrates the application of our technique to a case study. Furthermore we illustrate the tractability and accuracy of our solution approaches. Finally, Section \ref{sec:conclusion} provides a brief summary of our findings and direction for future research. 

%\jm{In Lit Review???}
%Campaign analysis, a method which applies models and techniques to answer questions about operational-level military operations, yields geopolitical insights and recommendations for senior decision makers \citep{teco21}. Campaign analysis applies scenarios --- plausible military settings that focus the military force --- to answer questions about military operations, e.g., \cite{shla16, maza19}. Campaign analysis is the most aggregated level of military modeling and simulation (M\&S) lying above mission, engagement, and engineering-level models in order of decreasing aggregation \citep{wade20}. Because it represents the operational level, campaign analysis influences wide-reaching decisions made at the strategic level. 

%\md{Do we care much about strategic in this paper?}. \jm{Yes, we care about strategic. Our model would not be useful as an operational-level planning tool - its main merit is quickly assessing strategic decisions with some operational context} 

%There are three levels of warfare: strategic, operational and tactical, where the operational level links the tactical employment of forces to national strategic objectives \citepalias{jp3-0}. At the operational level, Joint Force Commanders employ military forces to deter adversaries and support multinational partners at the geopolitical scale \citepalias{jp3-0}. Furthermore, operational warfare is the realization of many tactical-level decisions. Accordingly, we define \md{We don't usually introduce any definition in an introduction. The purpose of the introduction is to motivate and describe the main research question, and summarize the contributions} the military campaign as an operational-level representation of strategic investment in manning, training, and equipping as demonstrated through sequential tactical-level battles. With this definition in mind, we contend that the framework demonstrated in this paper links the three levels of warfare.

%Campaign analysis, a method which applies models and techniques to answer questions about operational-level military operations, yields geopolitical insights and recommendations for senior decision makers \citep{teco21}. Campaign analysis applies scenarios --- plausible military settings that focus the military force --- to answer questions about military operations, e.g., \cite{shla16, maza19}. Campaign analysis is the most aggregated level of military modeling and simulation (M\&S) lying above mission, engagement, and engineering-level models in order of decreasing aggregation \citep{wade20}. Because it represents the operational level, campaign analysis influences wide-reaching decisions made at the strategic level. Historic military campaigns such as Waterloo, Stalingrad, and Normandy all helped determine the outcome of major geopolitical conflicts. \md{I don't fully understand the point you are making here. The description is good, but after reading it, my question is: so what? That's because I cannot see the main thread and the link between the different pieces of information you are providing.}

%There are various models the military uses for campaign analysis. Staff members often rely on roundtable format, “political-military” (POL-MIL) games. These seminar style games are a great step towards identifying key elements of global competition. For operational problems, the military often relies on tabletop wargames to simulate combat operations. These games take days to assess military options against one adversary course of action and they are sensitive to player priorities, dominating personalities, and wargame rules. Simulation is another approach that produces results faster than a wargame. However, the campaign simulations often take months to build and can be  data intensive. Most importantly, all of these approaches take time and can only evaluate one scenario (e.g., force mix or starting conditions) at a time. \md{This previous paragraph is a bit in-between, in my opinion. In the literature review, you will want to explain in details what is usually done for campaign analysis (provide citations, and describe the limitations). Here, we only want a quick summary of the current approaches/limitations to introduce the gaps and motivate the research question you will work on.}

%Campaign analysis, through computer simulation or wargaming, helps assess geopolitical, strategic, and operational possibilities. These tools often link strategic-level decisions, such as investment in assets or activities, to operational-level impacts, e.g., \cite{muel16, flan19} \md{Do we care much about strategic in this paper?}. Furthermore, operational warfare is the realization of many tactical-level decisions. Accordingly, we define \md{We don't usually introduce any definition in an introduction. The purpose of the introduction is to motivate and describe the main research question, and summarize the contributions} the military campaign as an operational-level representation of strategic investment in manning, training, and equipping as demonstrated through sequential tactical-level battles. With this definition in mind, we contend that the framework demonstrated in this paper links the three levels of warfare.

%Although our framework may not provide the detail of a wargame or simulation \md{No need to downplay your model here. Focus on the positive side (and if there are limitations, you can frame them as a ``tradeoff'')}, it aims to yield quick, first-order assessments \md{This is about the impact/benefits of the model. I would keep this as the last set of contributions (you end the contributions by explaining who would benefit from your work (and how))}. This responsiveness allows the decision maker (DM) to evaluate a wide range of input scenarios. We seek to provide timely insights and first-order recommendations for strategic and operational decision making. 

%\jm{Gap in existing research}
%While the zero-sum stochastic game (often called a Markov game or competitive game) is a well established framework starting in the 1950s \citep{rag91, shap53} \md{Now you are going back to some quick lit review. This needs some reorganization}, the construct has not been extensively applied to military campaign analysis. To our knowledge, no existing research has framed an operational-level campaign as zero-sum game using our approach \md{To be merged with some of the limitations mentioned above. This statement can also be changed a bit. Instead of saying no campaign has been framed as a zero-sum game, you can instead say that there is no decision model for campaign analysis that considers the dynamic and stochastic aspect of military campaigns. (something like this). After the research question, you can then say you introduce the zero-sum game. It's better than saying (there is no zero-sum game, so we introduce a zero-sum game).}. Military analysts and operational-level planners have much to gain from this construct \citep{wash14} \md{Now this is again regarding who would benefit from it. (to be reoganized)}. Solving the game yields the Markov perfect equilibrium (MPE) policy and value, which provides insights to operational-level planners and campaign outcomes to strategic-level force developers. 

%\jm{Main research question} 
%At the outset we ask, can we model a military campaign as a stochastic game while maintaining sufficient resolution and computational efficiency for a responsive decision support system (DSS)? \md{Main research question will have to be adjusted. Something less technical that does not mention the stochastic game. (check Onkar's, Bastián's, or Lacy's) } We summarize this paper's contribution \md{That will need to be expanded. Please check my other papers to have a good idea on the amount of details to include}: 

%In this paper we build a military campaign with a special structure to reduce our state and action space. We solve or approximate the MPE policies and value through accelerated value iteration (AVI) and a heuristic we develop. 



==> Sec_2_Lit_Review_MathieuNotes.tex <==
%!TEX root = NRL Manuscript.tex
\section{Literature Review} \label{sec:lit}

%The two-player, zero-sum stochastic game, first developed in \cite{shap53}, is the sequential case where two players have completely opposed interests \citep{wash14}. 

\md{After reading this section, I believe it would be helpful for you to make a mental map of the points you are trying to make, including transitions between them. After reading this, a reader should have the answer to: What tools already exist in campaign analysis? How are stochastic games used in warfare and security in general? How is our paper different/new?}

Campaign analysis sits atop the military modeling hierarchy (Figure \ref{fig:hierarchy}). The campaign level trades off some detail to yield high-level, aggregated insights for military senior decision makers. \md{Is what we are doing really that high level?} The primary tools, wargaming and simulation, are ideal for their rigor and level of insight; yet they cannot assess many strategic decisions quickly. Subsequently, we seek to apply the more responsive zero-sum stochastic game to the campaign analysis domain.\md{Do you have any citations for wargames and simulation? It's important to have a paragraph dedicated to the current ways to analyze campaigns (wargames, simulation). And point some limitations/differences. Then, keep the transition to introduce stochastic games.}

While the stochastic game \md{Either ``the stochastic game framework'', or ``stochastic games''}has been applied in the overall military domain \md{Well, not for campaign analysis}, we assess that existing efforts are largely for the system/engineering or engagement levels with a few mission-level applications. \md{I would merge with the next paragraph}

%When viewing the military campaign as a chain of events (e.g., battles), the military analytic community often models these events separately through mission-level simulations. Then these mission results (e.g., battles) are compiled into the campaign level model.

\begin{figure}[H] 
\centering
\includegraphics[scale=.25]{img/hierarchy.PNG}
\caption{Department of Defense Modeling and Simulation Hierarchy \citep{wade20}}
\label{fig:hierarchy}
\end{figure}

% System/Engineering and Engagment-level

At the system/engineering and engagement levels, \cite{ho22} review many of stochastic game applications. For instance, \cite{bach11} and \cite{he21} study the competitive interaction between radars and jammers. \cite{deli17} study power allocation for a radar network against multiple jammers. Then, \cite{bogd18} and \cite{gu11} study target selection and tracking in radar networks. Finally, \cite{krish08} study transmission in ground sensor networks. The stochastic game is also used for the mission-level, which models military battles between forces. \cite{chang22} employ the partially observed stochastic game (POSG) to assess modern combat in Mosul. \cite{mce04} apply the stochastic game to air operation command and control. \md{All of this is good, but how do they relate with your model? In other words, why can't we utilize such models directly for your campaign problem? What main features are missing?}

    Stochastic games are used extensively for network interdiction problems \citep{wash95} \md{This paper is not a stochastic game. And I don't see the link with the previous paragraph. Where do these problems sit in Figure 1? Actually, they seem to be nonmilitary applications. You have to be explicit about it at the beginning of the paragraph to guide the reader. Here, you are talking about a broader class of security problems (but you need to differentiate with the previous paragraphs). Would you say that previous ones are for warfare and this is for security? Are any of these papers stochastic games for network interdiction? If not, you should not mention this field.}, whose attacker/defender paradigm avails to the military domain. For security and detection problems, \cite{bish21} and \cite{chang17} study the POSG in the development and food security domains respectively. Bishop employs the use of a ``precedence graph" for his problem, where players vie for control of ``artifact" nodes. \cite{wang23} and \cite{feng20} provide applications for power grid and network security. \cite{major02} applies the stochastic game to assessment of terrorism risk, with the defender goal of minimizing total expected loss. We adopt \cite{chang17} and \cite{bish21} to develop the command and logistics precedence structure and depict our game's state and action space \md{Is it exactly the same, or does it have some differences? Keep in mind that we have to answer the reviewers' main questions: How do we compare/differentate with the literature? Why can't we directly use one of these papers for our problem?}. Furthermore, our work aligns with \citeauthor{major02}'s \citeyear{major02} use of \textit{total expected loss} to represent the campaign risk\md{I find this to be a mild similarity, and would not necessarily mention it. Unless you argue otherwise}. \md{Instead, I would prefer if you focused on how our paper differs from these?}

The work of \cite{bier07} models \md{What type of model?}a defender who allocates defensive resources against locations where the adversary can attack. This closely relates to the Colonel Blotto game framework: zero-sum games with fixed resources and $n$ battlefields \citep{shub81,cough92}. The ``Colonel Blotto" game \citep{chowd13,wash14} has applications in the economic (e.g., development), political (e.g., campaigning), R\&D (e.g., securing patents), and the military domains \citep{kove21}. Opposing military commanders are allocated a finite number of forces (e.g., individual soldiers) that the commanders assign among a set of military objectives. The commanders act simultaneously, unaware of each other's decisions. The commander who places the highest number of forces on an objective gains that objective. While our game's players also assign resources by reinforcing or attacking military objectives, our problem is structured with subordinate commanders and logistics chains and the outcome of these battles is probabilistic \md{Note that there is a stochastic version of the colonel blotto game ``Strategy,  nontransitive  dominance  and  thee xponential distribution'', or ``ON ASYMPTOTIC STRATEGIES IN THE STOCHASTIC COLONEL BLOTTO GAME''. Success probability of player $i$ is $a_i/(a_1 + a_2)$ (where $a_i$ is the amount of resources)}. In totality, while existing military stochastic game research lends us valuable techniques, it does not capture the sequential, dynamic linkage between military events found in a military campaign. \md{This past sentence seems out of place. It is too generic to be here.}

\cite{haywood54}, who reviews the World War II Battles of the Bismarck Sea (U.S. versus Japan) and Avranches-Gap (Allies versus Germany), provides a launching point for our research. He portrays a military battle as one event, modeled as a matrix game. \cite{haywood54} uses the minimax solution to the matrix game as developed by \cite{vNeu28}. \cite{haywood54} demonstrates that portraying military decision making as a matrix game is a powerful decision support tool. \cite{cant03} and \cite{fox16} build on Haywood's work by applying a 10-step methodology or the analytic hierarchy process \md{What is the analytic hierarchy process? Is it standard?}to assign the utility of battle outcomes. While \cite{haywood54} provides a clear delineation of military decision making for the single-stage problem, the  work does not consider future military events that may occur as an outcome of one battle. Furthermore, \cite{haywood54} does not consider the dynamicity and stochasticity that occurs between military events \md{Past two sentences can be merged/shorten. The first one is kind of a subset of the second one}. So as \cite{shap53} adapts the single-stage, matrix game work of \cite{vNeu28} to the sequential, stochastic game setting \md{I'm not sure how I feel about this comparison. It is true, but I find it a bit grandiose :)}, we seek to adapt the single battle work of \cite{haywood54} to the sequential campaign setting. Linking these single-stage battles together through a transition model and the players' joint actions forms a sequential campaign.

\md{Organizational problem here. You can't go back to further limitations of the paper. I would regroup limitations together, and then explain how you extend all of them.}Additionally, while \cite{haywood54} assumes that a battle outcome given the players' joint action is deterministic, we contend that the outcome is uncertain. Furthermore, the outcome of one battle determines the future campaign state and subsequently the future battles that may occur \md{You are already saying this in the previous paragraph}. We must reflect military feasibility in our campaigns, so we decompose the campaign across the responsibility of multiple commanders who lead simultaneous battles within a logistics chain across military domains (e.g., land, air, space, and maritime) \md{Can you mention the probabilistic interdependencies across commanders? Unless you do it in the next paragraph}. \md{Past two paragraphs must be merged and possibly shortened.}

Overall, current stochastic game applications in the military domain consider one event \md{talking about one event is confusing, as it can relate to a static game.}, such as the interaction of a radar and jammer (system/engineering level), target selection (engagement level), or a military battle (mission level). Because these events are standalone, there is no connectivity between them for the campaign context. Instead, we envision a single event \md{I would not talk about single event} or battle as a matrix game, where each outcome determines the next state of the campaign. We can express the dynamic, sequential, and uncertain military campaign.
\md{This last paragraph is important. It should summarize your findings (without creating much repetition). And you should especially land your main point: To the best of our knowledge, this is the first stochastic game model of a military campaign.}

%From the network interdiction literature, we borrow the graph depiction to portray military objectives. Our state space depiction resembles \cite{bish21} and \cite{chang17}. Unlike \cite{bier07} we do not see one side as an attacker or defender, rather these roles change based on the objectives controlled.

%Campaign analysis trades off some resolution and detail for aggregation, to capture the vital parts of large military operations. Wargaming and computer simulation are currently used to explore this M\&S level. Potentially because of the intrinsic complexity and challenges in soliciting model inputs, we have not identified any existing methodologies that apply stochastic games to analytically model the sequential, multi-battle, military campaign.

%\md{Because you model supply lines. It's important to be precise in explaining how our model differs and what opportunities our model provide? What can you account for in your model that could not be considered in those other papers?}

%publish a review of military defense game theory applications and categorize the 29 papers they studied as ``resource allocation", ``information warfare", ``weapons control", and ``adversary monitoring". The reviewed papers generally focus on cyber security, sensing (e.g., radars), and tracking and sensor networks. \cite{ho22} further classify the research according to domain (e.g., land, sea), warfare type, number of players, and four game theory categorizations (e.g., zero-sum versus non-zero-sum). The taxonomy in \cite{ho22} would describe this \md{this as in ours?} paper as non-cooperative, simultaneous decision-making, discrete states and actions, and two-player, zero-sum. \cite{ho22} study two papers that meet this criteria:  Existing military papers that apply stochastic game models, tend to study engineering-level problems, such as the interaction between radars and jammers.


%Although we have not identified the stochastic game applied to the military campaign, \cite{haywood54} uses the minimax solution to the matrix game as in \cite{vNeu28} to model a military battle. Like the modeling and simulation hierarchy, we intend to adapt the mission-level work of \cite{haywood54} to the campaign setting.

%NEED TO DETERMINE IF THIS PARAGRAPH IS NECESSARY ANYWHERE
%The military campaign represents military conflict on the geopolitical scale. Inherently, at this decision-making level, game theory blends with human behavior in a field called behavioral game theory (BGT). In this field, payoffs are often asymmetrical and not purely competitive. \cite{cab20} apply BGT for military operational planning, arguing ``the lack of emphasis on players' humanity in traditional solution concepts has discouraged the application of game theory to the planning of military campaigns". \cite{schell61} creates the foundation for general sum games as they relate to international affairs expressing some challenges of the Cold War, such as a nuclear preemptive strike. We acknowledge the importance of human behavior in military campaigns; however, we assume that once military conflict begins the military objectives are zero-sum and military commanders act rationally to shape the campaign outcome. Indeed, the military needs to win in competition, so that competition does not become armed conflict \citepalias{hqda21}. Posturing the military force to best win in armed conflict as represented by the campaign MPE value represents a formidable deterrent to an adversary initiating conflict. In Sec. \ref{sec:case_study}, we demonstrate how military investment in assets and activities can shape a campaign's outcome, potentially deterring the adversary. Since assessing potentially multiple campaigns under differing scenarios is vital to assessing the competitive landscape, we view the zero-sum stochastic game model as a responsive, ideal selection.

%Dr. White: I think I follow this.  ‘Humanity’ and ‘human and occasionally irrational behavior’ are probably equivalent or close to it.  Game theory tells us what people (rational) should do rather than what they actually decide to do (BGT).  An interesting issue for human decision support (for a later paper perhaps).  Question: what if the adversary is occasionally irrational.  How does that affect our performance?  Does it improve our performance?

%\md{You have explained what they all consider, but my main question as a reader is: Among all these papers in this paragraph, none of them can be utilized for your problem? How is your model new (how does it differ)?}

%While the literature is well developed for the stochastic game, our contribution is towards the military campaign analysis domain, which offers a higher level of aggregation and insight than mission, engagement, and engineering models \citep{wade20} \md{We will turn this around. After you describe the current literature on military campaign analysis, you will highlight (and really emphasize) the main limitation: They don't consider dynamicity and stochasticity. And then you can potentially explain about two-person zero-sum games. Although I'll be honest, I'm not sure this will be needed. Some of this text on methods for solving 0-sum games can be included after you define the game in Section 3 (saying: Now we need to solve our game. Classical techniques involve x,y,z. However, we face limitations due to the size of the problem $->$ we need to exploit the problem's structure.}. 

%As Haywood demonstrates, the mental construct for military commanders to create matrix games by pitting their courses of action against their adversary's, is a useful planning exercise.

%\md{Some reoganization will indeed be needed. After you have introduced stochastic games (which will occur later in that section), you can then explain this paragraph, to mention it has only been employed in lower levels of military M\&S}

%The stochastic game has been applied to many tactical-level military applications \cite{mce04,chang22}, security problems \cite{wang23,feng20,bish21,chang17}, and network interdiction \cite{wash95}.

%\md{Some time is needed to figure out what information goes in this section. I'm not against briefly recapping zero-sum stochastic games here, but I think the order needs to change.

%1) You need to explain what models/approaches are used for campaign analysis.}

%One player seeks to minimize the overall payoff to the other player, while the other player seeks to maximize their payoff. The stochastic game, although initially developed separately, is a generalization of the Markov decision process (MDP) developed independently by Bellman, Howard, and others \citep{fila16,bell57,howard60} \md{The main question is: Is this whole paragraph needed? The goal of the literature review is to understand what has been done to tackle similar problems to the one you consider, and explain why you can't directly use them to solve your own problem. I don't believe a full explanation of zero-sum stochastic games here is needed.}. 



==> Sec_4_3_PNH.tex <==
%!TEX root = NRL Manuscript.tex



%\subsection{Lifted Value Function}
%
%Would in equilibrium the value function be a fixed point of another mapping where we first take the expectation over all other commanders?





\subsection{Commander's Focused Heuristic \md{To be changed}}


One of the main computational challenges in solving the stochastic game $\Gamma$ stems from the size of the players' action spaces. Indeed to achieve an MPE, it is often necessary for each player to coordinate orders between their commanders due to the interplay between axes via the transition probability function. For instance, controlling the airspace provides close air support (CAS) which greatly enables ground operations. A ground force may attempt to hold their current position until CAS is available. We illustrate this intuition with the following numerical example.



%
%In order to efficiently obtain good quality solutions, we develop a second solution approach tailored to the stochastic game $\Gamma$. In this heuristic, we decompose at each state the players' mixed strategies across commanders, and compute them asynchronously. 
%
%In equilibrium of $\Gamma$, coordinating is often necessary to achiev
%
%
%This section demonstrates that decentralized decision making does not necessarily yield the MPE strategy. This is due to the interplay between axes. Although objectives between axes are not connected by an edge, an objective in one axis may affect transition dynamics for an objective in another axis. For instance, controlling the airspace provides close air support (CAS) which greatly enables ground operations. A ground force may attempt to hold their current position until CAS is available. Building on this intuition, we demonstrate an analogous example.
%
%



%fast, we develop a second solution approach
%
%To speed up computations, we decompose at each state the players' mixed strategies across commanders, and compute them asynchronously.






\begin{example} Consider the campaign illustrated in Figure \ref{fig:ctrex1} with an air commander and a ground commander for each player. Each commander is managing an axis with two objectives. We suppose the initial state $s^\dag$ is given by $s_1^\dag = s_3^\dag = 1$ and $s_2^\dag = s_4^\dag = 2$, and the objective losses are given by $\ell_1 = \ell_2 = 0$, $\ell_3 = 1$, and $\ell_4 = 10$. The base attack and reinforce success probabilities are given by 



axis and a ground axis under the responsibility of an air and a grcomma



Suppose we have a campaign with an air commander and a ground commander. From the starting state, the player 1 ground commander (commander 2) may attack the next objective or reinforce the objective they control. The player 1 air commander (commander 1) is guaranteed to control the airspace (both objectives 1 and 2) on the next turn, assuring future success on ground operations. This example will demonstrate how the ground commander should not take the narrow-sighted decision to attack, and should instead reinforce and wait until air support is assured. We outline the campaign in Figure \ref{fig:ctrex1}. We assume that $\gamma$ approaches 1. The attack and reinforce probabilities from the starting state $s^\dag$ are $\rho^1_{1,s^\dag} = 0,\; \alpha^2_{1,s^\dag} = 0, \alpha^1_{1,s^\dag} = 1,\; \rho^2_{2,s^\dag} = 1,\; \rho^1_{3,s^\dag} = 0,\; \alpha^2_{3,s^\dag} = 0.5,\; \alpha^1_{4,s^\dag} = 0.2,\; \rho^2_{4,s^\dag} = 1$. These are also provided in the second frame in Fig. \ref{fig:ctrex1b}. Furthermore, from any $s \in \S$ where $s_1 = 1 = s_2$, for any feasible joint action, player 1 is guaranteed to succeed and player 2 is guaranteed to fail.

\begin{figure}[htbp]
\centering
\includegraphics[scale=.48]{img/ctrex1.png}
\caption{Counterexample to optimal decentralized decision making}
\label{fig:ctrex1}
\end{figure}

It is clear from Figure \ref{fig:ctrex1} that the ground commander should reinforce objective 3 rather than attack objective 4, yielding a lower expected total loss. However the narrowsighted decision for commander 2 is to attack objective 4. Now we assume that the ground commander has access to the state's true MPE value as depicted in Figure \ref{fig:ctrex1b}, and we demonstrate furnished with the MPE value, a commander may make the wrong decision when other axes are not taken into account. 
\begin{figure}[H]
\centering
\includegraphics[scale=.25]{img/ctrex1b.png}
\caption{MPE Value for States}
\label{fig:ctrex1b}
\end{figure}
\noindent
Recall that the optimality equation for a fixed action is:
\begin{equation*}
    V^{(t+1)}(s,a^1,a^2) \gets L(s) + \gamma  \sum_{s^\prime \in \S} P(s^\prime \ | \ s, a^{1},a^{2}) \cdot V^{(t)}(s^\prime)\
\end{equation*}
From this formula we create Table \ref{tbl:ctrex1}, which shows the single stage matrix game for the narrowsighted ground commanders.
\begin{table}[H]
\begin{center}
\caption{Matrix Game from DM Perspective}
\begin{tabular}{|p{2cm}|p{6cm}|p{6cm}|}
	\hline
	 & Attack 3 & Reinforce 4 \\
 	\hline
	Attack 4 & $10+(0.2)(0.5)0+(0.8)(0.5)20+ \newline (0.2)(0.5)1+(0.8)(0.5)26.5=28.7$   & $10+(0.2)0+(0.8)20 = 26$ \\
        \hline
	Reinforce 3 & $10+(1)(20)+(0)(26.5) = 30$ & $10+20=30$\\
	\hline
\end{tabular}
\label{tbl:ctrex1}
\end{center}
\end{table}

Under the narrow-sighted strategy, both ground commanders choose to attack. Yet, figure \ref{fig:ctrex1} shows that the player 1 ground commander's correct order is to reinforce objective 3. Instead the player 1 ground commander should reinforce until the air commander captures the airspace. 

\hfill$\triangle$

\end{example}

This section shows that the narrow-sighted strategy is not necessarily the MPE strategy in a combined multi-axes setting. Nonetheless, empirically, taking this narrowsighted decision can produces a good value approximation.



We do something in between: We decompose, but we compute them asynchronously, while accounting for the mixed strategy of the other commander.

Intuitively, this corresponds to strategies in a variant of the game $\Gamma$ where commanders cannot communicate with one another once the campaign has started. Thus, the policy profile is determined a priori, and commanders are aware of the mixed strategy they must implement (and the one implemented by the other commanders) at each state.

They know the whole state though
The main difference with the game $\Gamma$ is that they cannot coordinate the realization of the mixed strategy.





In order to efficiently obtain good quality solutions, we develop a second solution approach tailored to the stochastic game $\Gamma$. In this heuristic, we decompose at each state the players' mixed strategies across commanders, and compute them asynchronously. 


For each commander $c \in \C$, we denote by $\S^c = \{1,2\}^{\O^c}$ the set of substates for the objectives under their responsibility. We also denote by $\A^{i,c}_{s^c}$ the pure action set. A mixed strategy is then given by $\pi^{i,c}(s)$

$a^{i,c}$ is an action.
We denote by $a^{i,-c}$ the aggregate action over all commanders. Similarly for $\pi^{i,-c}(s)$.

Subgame $\Gamma(V^\prime,s,c,\pi^{1,-c}(s),\pi^{2,-c}(s))$.

%\begin{proposition}
%
%Let $V^\prime$ and $c$ be a commander managing a single axis $x$. If $V^\prime$ is isotone, then $\Gamma(V^\prime,s,c,\pi^{1,-c}(s),\pi^{2,-c}(s))$ has an equilibrium in pure strategies.
%
%\end{proposition}



We note that , and can serve as good (and fast) warm start solutions for the AVI algorithm.


\begin{algorithm}[htbp]
\caption{Heuristic} \label{alg:heuristic}
\normalsize
\SetArgSty{textnormal}
\SetKwInOut{Parameters}{Parameters}
\SetKwInOut{Input}{Input}
\SetKwInOut{Output}{Output}
\SetKwIF{nlIf}{ElseIf}{Else}{if}{then}{else if}{else}{\nl}
\SetKwRepeat{Do}{do}{while}
%\Parameters{Integers $k_1$, $k_2$, and $b$, positive number $\varepsilon$}
\Input{Game $\Gamma = \langle\S,(\A^1,\A^2),P,L,\gamma\rangle$ and optimality gap\md{scalar/stopping criterion} $\epsilon \in \mathbb{R}_{>0}$}
\Output{\md{to change}$\epsilon/2-$approximate game value $V^{(t)} \in \mathbb{R}^\S$ and $\epsilon$-MPE $(\pi^{1^\prime},\pi^{2^\prime}) \in \Delta^1\times \Delta^2$}
\BlankLine
%\nl Initialize: Reduced Cost $ (\Bar{c})_{p \in \mathcal{P}} \gets \, -M , \quad $ Parameter $(\kappa)_{p \in \mathcal{P}} \gets 0$ \;
%\nl Path set as warm-start $\tilde{\Lambda} \gets \tilde{\Lambda} \setminus \{\lambda \in \tilde{\Lambda} |  i \in \lambda \cap \mathcal{Y}^{0} \}$  and define $\mathcal{L}_{path}(\mathcal{Y}^{0},\mathcal{Y}^{1},\tilde{\Lambda})$ \md{Do this when assigning to child node} \;

$t \gets 0$\;

$\widehat{V}^{(t)} \gets L$\;

Randomly initialize $\widehat{\pi}^{i,c}(s) \in \Delta(\A^{i,c}_s)$, $\forall i \in \{1,2\}, \ \forall c \in \C, \ \forall s \in \S$\;


\Do{$\| \widehat{V}^{(t)} - \widehat{V}^{(t-1)}\|_{\infty} > \epsilon (1-\gamma)/(2\gamma)$}{


\For{every $c \in \C$}{

$t \gets t+1$\;

\For{every $s \in \S$}{


$\widehat{R}(\widehat{V}^{(t-1)},s,c,a^{1,c},a^{2,c}) \gets L(s) + \gamma  \cdot\sum_{s^{c^\prime} \in \S^c} \prod_{o \in \O^c} p_o(s^\prime_o \, | \, s,a^{1,c},a^{2,c}) \cdot \mathbb{E}_{a^{1,-c}\sim\pi^{1,-c}(s),a^{2,-c}\sim\pi^{2,-c}(s^{c^\prime}),}[\sum_{s^{-c^\prime}}\widehat{V}^{(t-1)}(s^{c^\prime},s^{-c^\prime})], \ \forall (a^1,a^2) \in \A^1_s \times \A^2_s$\;

$(\widehat{V}^{(t)}(s),(\widehat{\pi}^{1,c}(s),\widehat{\pi}^{2,c}(s))) \gets $ AZS($s,\A^{1,c}_s,\A^{2,c}_s,R(\widehat{V}^{(t-1)},s))$\;

}


}}
\nl \KwRet{$\widehat{V}^{(t)}$, $(\widehat{\pi}^{1},\widehat{\pi}^{2})$ }
\end{algorithm}


Policy evaluation:





A heuristic that exploits a narrow-sighted intuition can provide further computational savings beyond AVI. Like AVI, our Commander's Focused Heuristic (CFH) relies on iteration for value update, but applies an analytic solution to select each axis action and subsequently reduce the joint action set to create a smaller single-stage matrix game. We now provide some foundation for the CFH.

%\begin{definition} \label{def:vec_order}
%    For two states of length $|\mathcal{O}|$, $s \prec s'$ (resp. $s \succ s'$) if $s \neq s'$ and $s_o \leq s'_o$ (resp. $s_o \geq s'_o$) \text{ for every } $o \in \mathcal{O}$. %In this case $s$ dominates $s'$ from the player 1 perspective. We say $s \succ s'$ if $s \neq s'$ and $s_o \geq s'_o$ for every $o \in \mathcal{O}$. In this case $s$ dominates $s'$ from the player 2 perspective.
%\end{definition}

%\begin{proposition} \label{claim:partial_ordering}
%    $V(\bm{s}') \leq  V(\bm{s})$ for $\bm{s}' \prec \bm{s}$.
%\end{proposition}
%
%\jm{we prove this in the annex}

%\subsubsection{CFH Development: One-axis Game} \label{sec:PNH1}
%
%We now show that a saddle point always exists for a one-axis game. As we show in the Proposition \ref{prop:reduce} proof, the one-axis decision for both players is trivial when $\tau(x) \neq \textit{pf}$. So we establish a game for $\tau(x,s) = pf$, where each player may \textit{atk} or \textit{rfc}. We let $R^x$ be the matrix game for the axis $x$ game for an arbitrary state.

%Defined from Player 1's perspective, there are four outcomes to a \textit{pf}-classified axis game: \textit{win, lose, swap, and draw}. \textit{Win} occurs when Player 1 gains an objective but Player 2 does not. \textit{Lose} occurs when Player 2 gains an objective but player 1 does not. \textit{Swap} occurs when both players attack and are successful, thereby \textit{swapping} objectives. \textit{Draw} occurs when neither player gains an objective and the state remains the same. All four outcomes are possible when both players attack. When player 1 reinforces, \textit{draw} or \textit{lose} may result. When player 2 reinforces, \textit{draw} or \textit{win} may result. 

%Suppose the current state is $s$, then set of all possible subsequent states from $s$ is $s_{win}$, $s_{lose}$, $s_{swap}$, and $s_{draw} = s$. We abbreviate the value of each of these states as $V_{win}$, $V_{lose}$, $V_{swap}$ and $V_{draw}$. The probabilities of each outcome may be expressed in terms of $\alpha^i$: the probability of player $i$ successful attacking and $\rho^i$ the probability of player $i$ unsuccessfully reinforcing.

%\begin{table}[H]
%\begin{center}
%\caption{Probabilities of Outcome for Single-Axis Game $R^x$}
%\begin{tabular}{|c|c|c|c|c|}
%	\hline
%Joint Action ($a$) & Win & Lose & Swap & Draw \\ \hline
%{(\textit{atk,atk})} & $\alpha^1 (1-\alpha^2)$ & $(1-\alpha^1) \alpha^2$ & $\alpha^1 \alpha^2$ & $(1-\alpha^1)(1-\alpha^2)$ \\ \hline
%{(\textit{atk,rfc})} & $\alpha^1 \rho^2$ & 0 & 0 & $(1-\alpha^1) + \alpha^1(1-\rho^2)$ \\ \hline
%{(\textit{rfc,atk})} & 0 & $\rho^1 \alpha^2$ & 0 & $(1-\alpha^2) + (1-\rho^1)\alpha^2$ \\ \hline
%{(\textit{rfc,rfc})} & 0 & 0 & 0 & 1 \\ \hline
%\end{tabular}
%\label{table:s_prime}
%\end{center}
%\end{table}
%
%%%%%%%%%%%%% THIS KIND OF SIMPLIFIES THE MATH BUT DOESNT REALLY HELP US %%%%%%%
%We now apply the fact that the NE for a matrix game is preserved under a linear transformation such as the subtraction of a constant \cite{espi20, wash14}. Suppose we have the vector of state values: $\bm{U}$. From Definition \ref{def:vec_order} and Claim \ref{claim:partial_ordering}, it follows that the smallest subsequent state value in $\mathcal{S}'$ is $U(\bm{s}_{win})$, so we let $U(\bm{s}_{win})$ be the constant we subtract from every possible $\bm{s}' \in \mathcal{S}'$: 

%\begin{align*}
%    \delta_{win} &= U(\bm{s}_{win}) - U(\bm{s}_{win}) = 0 \\
%    \delta_{lose} &= U(\bm{s}_{lose})-U(\bm{s}_{win}) \\
%    \delta_{swap} &= U(\bm{s}_{swap})-U(\bm{s}_{win}) \\
%    \delta_{draw} &= U(\bm{s})-U(\bm{s}_{win})
%\end{align*}

%We apply $\delta_{win}, \delta_{lose}, \delta_{swap}, \text{ and } %\delta_{draw}$ along with Table \ref{table:s_prime} to create $\bm{G}^x$:

%\begin{table}[H]
%\begin{center}
%\caption{$R^x$}
%\begin{tabular}{|p{2cm}|p{6cm}|p{6cm}|}
%	\hline
%	 & 1: \textit{atk} & 2: \textit{rfc}  \\
% 	\hline
%	1: \textit{atk} & $\alpha^1(1-\alpha^2)V_{win} + (1-\alpha^1)\alpha^2V_{lose} + \alpha^1 \alpha^2 V_{swap} + (1-\alpha^1)(1-\alpha^2)V_{draw}$ & $\alpha^1\rho^2 V_{win} + (1-\alpha^1\rho^2) V_{draw}$ \\
%        \hline
%	2: \textit{rfc} & $(1-\rho^1\alpha^2)V_{draw} + \rho^1\alpha^2 V_{lose}$& $V_{draw}$  \\
%	\hline
%\end{tabular}
%\label{table:2}
%\end{center}
%\end{table}
%
%May have to prove claim 1 at some point, perhaps in appendix

%In Table \ref{table:2} we assign natural numbers to each player action (1=\textit{atk},2=\textit{rfc}) and let $R^x(a^1,a^2)$ denote the $R^x$ element for joint action $(a^1,a^2)$.  Because $\rho^1,\rho^2,\alpha^1,\alpha^2, \text{ and } V_{draw} \geq V_{win}$, $R^x(2,2) \geq R^x(1,2)$, with strict equality holding when $\rho^1,\rho^2,\alpha^1,\alpha^2, \text{ and } V_{draw} > V_{win}$. Next we see that because $V_{lose} \geq V_{draw}$ that $R^x(2,1) \geq R^x(2,2)$ with strict equality holding when $V_{lose} > V_{draw}$. Thus: 
%
%\begin{equation} \label{eq:Gorder}
%  R^x(2,1) \geq R^x(2,2) \geq R^x(1,2)  
%\end{equation}

%\md{Main idea: show that (rfc,rfc) is not an equilibrium.}

%We now show that the saddle point exists and provide the equation to find the saddle point.

%\begin{proposition} \label{lem:saddle}
%    A pure saddle point always exists for $R^x$.
%\end{proposition}
%
%%\jm{FIX THIS NOTATION: https://math.stackexchange.com/questions/679880/existence-of-saddle-point-of-a-matrix-shapleys-theorem}
%\jm{Move to annex when ready}
%\proof{Proof of Proposition \ref{lem:saddle}.}
%We know a saddle point exists for $R^x$ if:
%    \begin{equation}
%        \min_{a^1\in\{\textit{atk,rfc}\}} \max_{a^2\in\{\textit{atk,rfc}\}}R^x(a^1,a^2) = \max_{a^2 \in\{\textit{atk,rfc}\}} \min_{a^1 \in\{\textit{atk,rfc}\}} R^x(a^1,a^2)
%    \end{equation}
%
%%\begin{equation} \label{eq:puresaddle}
%%\min\{\max( \bm{G}_{1,1}, \bm{G}_{1,2}),\max( \bm{G}_{2,1}, \bm{G}_{2,2})\} = \max\{\min( \bm{G}_{1,1}, %\bm{G}_{2,1}),\min( \bm{G}_{1,2}, \bm{G}_{2,2})\}
%%\end{equation}
%
%\textit{Case 1:} $ R^x(1,1)\geq  R^x(2,1)$\\
%$R^x(1,1)$ and $ R^x(2,1)$ are the maximizing arguments for each row based on the case assumption and transitivity and Eq. \ref{eq:Gorder} respectively. $ R^x(2,1)$ is a minimizing argument among these two. $ R^x(2,1)$ and $ R^x(1,2)$ are minimizing arguments for each column based on the case assumption and Eq. \ref{eq:Gorder} respectively. $R^x(2,1)$ is a maximizing argument for these two minimizing arguments based on our case assumption and transitivity with \ref{eq:Gorder}. Therefore, $ R^x(2,1)$ is a saddle point.
%
%\textit{Case 2:} $ R^x(1,1) <  R^x(2,1)$\\
%Either $ R^x(1,1)$ or $ R^x(1,2)$ is the maximizing argument for row 1, since we do not know which is larger. $ R^x(2,1)$ is a maximizing argument for the second row by \ref{eq:Gorder}. A minimizing argument among these is $\max( R^x(1,1), R^x(1,2))$ since we know that $ R^x(1,2) \leq  R^x(2,1)$ and $ R^x(1,1) <  R^x(2,1)$. $ R^x(1,1)$ and $ R^x(1,2)$ are minimizing column arguments by the case assumption and \ref{eq:Gorder}. The maximizing argument of these is $\max(R^x(1,1), R^x(1,2))$. Thus the saddle point is $\max(R^x(1,1), R^x(1,2))$.
%
%\hfill\Halmos
%\endproof

%We denote this saddle point, the joint, deterministic decision: $\hat{d}_x = (\hat{d}^1_x,\hat{d}^2_x)$. When $\rho_1,\rho_2,\alpha_1,\alpha_2, \text{ and } V_{draw} > V_{win}$, it follows that $\hat{d}_x$ will never be (\textit{rfc,rfc}) and the analytic solution may be found:
%\[
%	\hat{d}_x=\begin{cases}
%             (\textit{rfc,atk}) &\text{if    } \alpha^1(1-\alpha^1)V_{win} + (1-\alpha^1)\alpha^2V_{lose} + \alpha^1 \alpha^2 V_{swap} + (1-\alpha^1)(1-\alpha^2)V_{draw} \geq \\
%             &\alpha^1\rho^2 V_{win} + (1-\alpha^1\rho^2) V_{draw} \\
%		(\textit{atk,rfc}) &\text{elif } \alpha^1(1-\alpha^1)V_{win} + (1-\alpha^1)\alpha^2V_{lose} + \alpha^1 \alpha^2 V_{swap} + (1-\alpha^1)(1-\alpha^2)V_{draw} < \\
%  &\alpha^1\rho^2 V_{win} + (1-\alpha^1\rho^2) V_{draw} \\
%		(\textit{atk,atk}) &\text{else }\\
%	\end{cases}
%\]
%\jm{We dont need the monotonicity result for this, we used that result for \textit{rfc,rfc} elimination}

%MILITARY NARRATIVE, IF NECESSARY
%\jm{Do you think this below para is necessary Mathieu? If so, I probably need to make it sound a tad better}
%In military terms, the relationship of node importance and the probability of successfully attacking or reinforcing the nodes determines which action the commander should take. Reinforcing is akin to the military notion of \textit{consolidating gains} and attacking is akin to the notion of \textit{seizing the initiative}. If the importance of the currently controlled objective times the probability of losing the objective despite reinforcing is lower than the difference in importance of the controlled objective times the adversary attack probability and the importance of the uncontrolled objective times our attack probability, then the commander should consolidate gains. If the opposite relationship holds true, the commander should seize the initiative.

%\subsubsection{CFH Development: Multiple-axis, One-commander Game} \label{sec:PNH2}
%Now we expand to the setting where a single commander $c$ is responsible for multiple axes. In the two-axis, one-commander game presented in Figure \ref{fig:2ax}, $|\mathcal{C}|=1$ and $|\X| = |\X_c| = 2$. The two axes are denoted $x$ and $y$, and the matrix game is denoted $R^{x+y}$. 
%
%\begin{figure}[H]
%\centering
%\includegraphics[scale=.7]{img/two_axis.png}
%\caption{Two Axes, One Commander Game}
%\label{fig:2ax}
%\end{figure}
%The commander may give up to one \textit{atk} or \textit{rfc} order. While in $R^x$, the deterministic, joint strategy always exists, the players may take a mixed strategy in $R^{x+y}$. There are four actions per player and 16 joint actions for $R^{x+y}$. Table \ref{table:twoaxis} presents the full joint action space ($\mathcal{A}_{x+y}$) for $R^{x+y}$. We will use this table to prove Lemma \ref{lem:twoaxis}.
%
%\begin{table}[h]
%\begin{center}
%\caption{Matrix Game for Two Axis}
%\begin{tabular}{|c|c|c|c|c|}
%	\hline
%	 & 1: \textit{atk} $x$ & 2: \textit{rfc} $x$ & 3: \textit{atk} $y$ & 4: \textit{rfc} $y$ \\
% 	\hline
%	1: \textit{atk} $x$ & $R^{x+y}(1,1)$ & $R^{x+y}(1,2)$ & $R^{x+y}(1,3)$ & $R^{x+y}(1,4)$ \\
%        \hline
%	2: \textit{rfc} $x$ & $R^{x+y}(2,1)$ & $R^{x+y}(2,2)$ & $R^{x+y}(2,3)$ & $R^{x+y}(2,4)$  \\
%	\hline
%        3: \textit{atk} $y$ & $R^{x+y}(3,1)$ & $R^{x+y}(3,2)$ & $R^{x+y}(3,3)$ & $R^{x+y}(3,4)$  \\
%        \hline
%        4: \textit{rfc} $y$ & $R^{x+y}(4,1)$ & $R^{x+y}(4,2)$ & $R^{x+y}(4,3)$ & $R^{x+y}(4,4)$  \\
%        \hline
%\end{tabular}
%\label{table:twoaxis}
%\end{center}
%\end{table}
%
%\jm{I do not believe this violates Thm. 1 and Prop. 1. In the proof we limited to $a^1 = \textit{rfc } o^\dag$ as an upper bound on $V(s,a)$. If $V(s,a^1=\textit{atk } o^{\dag},a^2) < V(s,a^1=\textit{rfc } o^\dag,a^2)$, then $V(s,a^1 =\textit{rfc } o^{\dag},a^2)$ remains an upper bound. 
%
%Additionally, $a^1=\textit{rfc } o^\dag$ is not eliminated from the single-axis action set a priori. It is still given consideration and if it is bested by $a^1=\textit{atk } o^\dag$, then it is not needed in the multiple axis case. I understand then the rationale still holds: if you would not reinforce in the single axis case, you would not reinforce when a commander has multiple axes.}
%
%
%\begin{proposition} \label{lem:twoaxis}
%    If Player $i$  does not select \textit{rfc} for $R^x$ then Player $i$ should not select \textit{rfc x} for $R^{x+y}$: $\hat{d}^i_x \neq \textit{rfc}$ for $R^x \implies \textit{rfc x} \notin \mathcal{A}^i_{x+y}$ for $R^{x+y}$.
%\end{proposition}
%
%\jm{Move to appendix when ready}
%\proof{Proof of Proposition \ref{lem:twoaxis}.}
%
%     We seek to find the conditions where a row action of \textit{rfc x} may be eliminated from $R^{x+y}$. An action $a$ may be eliminated if one different action $a'$ is more or equally preferable \textit{against every opposing player action}.
%     
%     Without loss of generality we compare Player 1's actions for axis $x$ only (the first two rows of Table \ref{table:twoaxis}). Thus we compare $R^{x+y}(1,1)$ to $R^{x+y}(2,1)$, $R^{x+y}(1,2)$ to $R^{x+y}(2,2)$, $R^{x+y}(1,3)$ to $R^{x+y}(2,3)$, and $R^{x+y}(1,4)$ to $R^{x+y}(2,4)$, to see under what conditions \textit{atk x} is preferable to \textit{rfc x}, thereby allowing us to eliminate \textit{rfc x}. We let $\alpha^i_x$ and $\rho^i_x$ be the probability that player $i$ successfully \textit{atk x} or unsuccessfully \textit{rfc x} respectively.
%
%     We let $V_{outcome1, outcome2}$ be the value after transitioning to a state where axis $x$ has $outcome1$ and axis $y$ has $outcome2$. For instance $V_{win,lose}$ is the value of the state where player 1 \textit{wins} in axis $x$ and \textit{loses} in axis $y$. Furthermore, we know that every $V_{outcome1, outcome2}$, $\alpha^i_x$, $\alpha^i_y$, $\rho^i_x$, and $\rho^i_y \geq 0$. 
%     
%     %For all comparisons, it may be preferable for player 1 to perform an axis 2 action, but this analysis does not add to the proof, so we only consider the first two row actions.
%
%\textit{Comparison 1}
%\begin{align*}
%    R^{x+y}(1,1)&= \alpha^1_x(1-\alpha^2_x)V_{win,draw}+\alpha^2_x(1-\alpha^1_x)V_{lose,draw}+\alpha^1_x\alpha^2_x V_{swap,draw}+(1-\alpha^1_x)(1-\alpha^2_x)V_{draw,draw}\\ 
%    R^{x+y}(2,1)&= \rho^1_x\alpha^2_x V_{lose,draw}+\alpha^2_x(1-\rho^1_x) V_{draw,draw}
%\end{align*}
%We cannot eliminate \textit{rfc x} without knowing more information about $\alpha^1_2$, $\alpha^2_1$, and $\rho^1_1$.
%
%\textit{Comparison 2}
%\begin{align*}
%    R^{x+y}(1,2)&= \alpha^1_x\rho^2_x V_{win,draw}+\alpha^1_x(1-\rho^2_x)V_{draw,draw}\\
%    R^{x+y}(2,2)&= V_{draw,draw}
%\end{align*}
%%\jm{Need our claim result of course}
%Because $s_{win,draw} \prec s_{draw,draw}$ we conclude that $V_{win,draw}\leq V_{draw,draw}$ and so $R^{x+y}(1,2)\leq R^{x+y}(2,2)$. Thus if Player 2 selects \textit{rfc x}, it is at least equally preferable for Player 1 to select \textit{atk x}.
%
%%Technically if all the probabilities are 0 it is not "preferable"
%
%\textit{Comparison 3}
%\begin{align*}
%    R^{x+y}(1,3)&= \alpha^1_x\alpha^2_y V_{win,lose}+\alpha^1_x(1-\alpha^2_y) V_{win,draw}+(1-\alpha^1_x)\alpha^2_y V_{draw,lose}+(1-\alpha^1_x)(1-\alpha^2_y) V_{draw,draw}\\ 
%    R^{x+y}(2,3)&= \alpha^2_y V_{draw,lose}+(1-\alpha^2_y) V_{draw,draw}
%\end{align*}
%If Player 2 selects \textit{atk y}, then player 1 selecting \textit{rfc x} will have no effect. $V_{win,lose}\leq U=V_{draw,lose}$ and $V_{win,draw}\leq V_{draw,draw}$, so $R^{x+y}(1,3)\leq R^{x+y}(2,3)$. Thus it would be at least equally preferable for Player 2 to \textit{atk x}. 
%
%\textit{Comparison 4}
%\begin{align*}
%    R^{x+y}(1,4)&= \alpha^1_x V_{win,draw}+(1-\alpha^1_x) V_{draw,draw}\\
%    R^{x+y}(2,4)&= V_{draw,draw}
%\end{align*}
%Here, $R^{x+y}(1,4)\leq R^{x+y}(2,4)$ so if Player 2 selects \textit{rfc y}, it is at least equally preferable for Player 1 to \textit{atk x}.
%
%In comparisons 2-4, it is at least equally preferable for player 1 to \textit{atk x} rather than \textit{rfc x}. 
%
%%Actions on axis $y$ may be even more preferable, but this assessment is unnecessary for this proof. 
%
%Now, we return to comparison 1. Only, when  $\alpha^1_x(1-\alpha^2_x) V_{win,draw}+\alpha^2_x(1-\alpha^1_x) V_{lose,draw}+\alpha^1_x\alpha^2_x V_{swap,draw}+(1-\alpha^1_x)(1-\alpha^2_x) V_{draw,draw} > 
%\rho^1_x \alpha^2_x V_{lose,draw}+\alpha^2_x(1-\rho^1_x) V_{draw,draw}$, is \textit{atk x} not preferable to \textit{rfc x}. Because axis $y$ will remain the same under these joint actions and $V_{outcome1,draw} = V_{outcome1}$, we only consider the state transition of $x$. Comparison 1 now follows the case 1 comparison for Proposition \ref{lem:saddle}. So \textit{rfc x} is only preferable to \textit{atk x} when: $\alpha^1_x(1-\alpha^2_x) V_{win}+\alpha^2_x(1-\alpha^1_x) V_{lose}+ \alpha^1_x \alpha^2_x V_{swap}+(1-\alpha^1_x)(1-\alpha^2_x) V_{draw} > \rho^1_x\alpha^2_x V_{lose}+\alpha^2_x(1-\rho^1_x)V_{draw}$ which is the same condition found in Section \ref{sec:PNH1}. Thus, only if player 1 selects reinforce in $R^x$, should \textit{rfc x} be considered as part of a mixed strategy in $R^{x+y}$. Otherwise \textit{rfc x} may be eliminated from the action set for $R^{x+y}$. 
%
%\hfill\Halmos
%
%\endproof

%Recalling the calculations for $\delta_{outcome}$ from Section \ref{sec:PNH1}, we arrive at the same criteria as the single axis game: $(1-\alpha^1_x)\alpha^2_x\delta_{lose} + \alpha^1_x \alpha^2_x \delta_{swap} + (1-\alpha^1_x)(1-\alpha^2_x)\delta_{draw} > (1-\rho^1_x\alpha^2_x)\delta_{draw} + \rho^1_x\alpha^2_x \delta_{lose}$. 

%Since we did not consider Player 1 axis $y$ actions in the proof, it is apparent that that Lemma \ref{lem:twoaxis} extends to any multiple-axis game: $R^{x+\mathcal{X} \setminus x}$. However the Proposition \ref{lem:twoaxis} implication does not apply to the \textit{atk x} action. Selecting \textit{rfc} for $R^x$ does not eliminate \textit{atk x} from consideration in $R^{x+y}$. For a historical example, the Maginot Line was established in the interwar period before World War II \citep{hist09}. Despite the efforts of the French military to reinforce their defenses along this one axis, the attacking Germans attacked along another axis through Belgium. An opponent may bypass a reinforced axis and attack another axis. Thus, if $\hat{d}^i_x = \textit{rfc}$ for $R^{x}$, then player $i$ must consider both \textit{rfc x} and \textit{atk x} for $R^{x+y}$. However, if $\hat{d}^i_x = \textit{atk}$ for $R^{x}$, player $i$ only needs to consider \textit{atk x} for $R^{x+y}$. 

\subsubsection{CFH Overview} \label{sec:PNH3}

Next, we tie together the previous results to finalize the CFH algorithm. The algorithm does not necessarily yield the optimal result because it is based on the assumption that $\mathcal{X} \setminus x$ remains the same when $\hat{d}_x$ is found. However, the state of $\mathcal{X} \setminus x$ changes simultaneously to $x$. Because these axes are probabilistically intertwined, other axes need to be taken into account to find the correct MPE solution. \md{I think this needs to be clarified, I believe it's about axes under the responsibility of other commanders, as you illustrate next.} As a military example: a ground commander may continue to reinforce a military objective until the adjacent air commander controls the airspace and is able to provide close air support. Only then, after success is more assured, will the commander attack another ground objective.

During the CFH algorithm, we complete three major steps for each state during every iteration. For every $x \in \mathcal{X}$, we find $\hat{d}_x$ from the Section \ref{sec:PNH1} results. Then from $\hat{d}_x$ for every $x \in \mathcal{X}$ we create the \textit{reduced set of joint actions} applying Section \ref{sec:PNH2}. We call this reduced action set $\hat{\mathcal{A}}_s$. From $\hat{\mathcal{A}}_s$, we create the reduced game $\hat{R}(v^{(t-1)},s)$ which we solve using the same procedure as AVI. We present the following steps for an arbitrary state $s$.

\textit{Step 1 (Narrow-sighted step):} Find the saddle point $\hat{d}_{x,s}$ for every $x \in \X$. $\hat{d}_{x,s}$ is (\textit{rfc,atk}) when $\tau(x,s) = \textit{c1}$, (\textit{atk,rfc}) when $\tau(x,s) = \textit{c2}$, and (\textit{atk,atk}) when $\tau(x,s) = \textit{sf}$. Thus, $\hat{d}_{x}$ only needs to be found when $\tau(x,s) = \textit{pf}$.

\textit{Step 2:} Create $\hat{\mathcal{A}}_s$ from $\hat{d}_{x,s}$ for every $x \in \X$. Although we can quickly find $\hat{d}_{x,s}$ for each $x \in \mathcal{X}$, $c$ must create a mixed strategy for a commander $c$ when $|\X_c| > 1$. From $\hat{d}_{x,s}$ for every $x \in \mathcal{X}_c$ we build the reduced action set for each commander $c \in \mathcal{C}$ from the rules prescribed in Section \ref{sec:PNH2}. The player $i$, commander $c$ reduced action set we call $\hat{\mathcal{D}}^{i,c}_s$. The Cartesian product of $\hat{\mathcal{D}}^{i,c}_s$ for every $c \in \mathcal{C}$ we denote $\hat{\mathcal{A}}^i_s$. This procedure is reviewed in Algorithm \ref{alg:getahat}.

%Furthermore, if $\hat{d}^i_{\bm{s},_x} = \textit{rfc}$, there is no guarantee that \textit{atk x} will not be part of the mixed strategy. However, we will show in Section \ref{sec:heu3} that if $\hat{d}^i_{\bm{s},_x}=atk$, then \textit{rfc} will not be part of the PNH combined action for $x$. With these rules, we create the reduced player $i$ action set: $\hat{\mathcal{A}}^i_{\bm{s}}$. In Algorithm \ref{alg:getahat}, we outline the procedure that yields $\hat{\mathcal{A}}^i_{\bm{s}}$. We will use $\mathcal{D}^{i,c}$ to denote the PNH action set for player $i$, commander $c$.

\begin{algorithm}[htbp]
\caption{Routine: Get $\hat{\mathcal{A}}^i_s$} \label{alg:getahat}
\normalsize
\SetArgSty{textnormal}
\SetKwInOut{Parameters}{Parameters}
\SetKwInOut{Input}{Input}
\SetKwInOut{Output}{Output}
\SetKwIF{nlIf}{ElseIf}{Else}{if}{then}{else if}{else}{\nl}
\SetKwRepeat{Do}{do}{while}
%\Parameters{Integers $k_1$, $k_2$, and $b$, positive number $\varepsilon$}
\Input{List of deterministic, one-axis decisions $(\hat{d}^i_{1,s}, \hat{d}^i_{2,s}, ... , \hat{d}^i_{|\X|,s})$}
\Output{Reduced Heuristic Action Set: $\hat{\mathcal{A}}^i_s$}
\BlankLine

\For{every $c \in \mathcal{C}$}{
    \If{$|\X_{c}|=1$}{$\hat{\mathcal{D}}^{i,c}_s= \{\hat{d}^i_{x,s}\}$}
    \Else{\For{$k,x \in$ \textit{Enumerate} $\X_c$} {$\hat{\mathcal{D}}^{i,c}_{k,s} = \{none,\hat{d}^i_{x,s}\}$
            \If{$\hat{d}^i_{x,s} = \textit{rfc}$ and $\tau(x,s)=\textit{pf}$}{Append \textit{atk} to $\hat{\mathcal{D}}^{i,c}_{k,s}$}
    }
    }
}
$\hat{\mathcal{A}}^i_s \gets \hat{\mathcal{D}}^{i,1}_s \times \hat{\mathcal{D}}^{i,2}_s \times ... \times \hat{\mathcal{D}}^{i,|\mathcal{C}|}_s \gets \text{Cartesian product of commander reduced action sets}$

\nl \KwRet{$\hat{\mathcal{A}}^i_s$}
\end{algorithm}

\textit{Step 3: Create reduced game $\hat{R}(V^{(t-1)},s)$ and find $\hat{\pi}(s)$.} Now given $\hat{\mathcal{A}}_s$ through Algorithm \ref{alg:getahat} and the previous value, we create the PNH reduced game: $\hat{R}(V^{(t-1)},s)$. Solving $\hat{R}(V^{(t-1)},s)$ gives the CFH strategy which we denote $\hat{\pi}(s)$. CFH completes iterations faster than AVI due to the reduced action set.

%We now outline the PNH algorithm and restore the state to the notation; for instance $\hat{\pi}(\bm{s})$ denotes the PNH policy for state $\bm{s}$.

\begin{algorithm}[htbp]
\caption{Partially Narrow-sighted Heuristic} \label{alg:PNH}
\normalsize
\SetArgSty{textnormal}
\SetKwInOut{Parameters}{Parameters}
\SetKwInOut{Input}{Input}
\SetKwInOut{Output}{Output}
\SetKwIF{nlIf}{ElseIf}{Else}{if}{then}{else if}{else}{\nl}
\SetKwRepeat{Do}{do}{while}
%\Parameters{Integers $k_1$, $k_2$, and $b$, positive number $\varepsilon$}
\Input{Game $\Gamma = (\S,(\A^1,\A^2),P,\ell,\gamma)$, initial vector $V^{(0)} \in \mathbb{R}^\S$, max iterations: $T$}
\Output{Game value approximation: $\hat{V}^{(T)}$}
\BlankLine

\For{every $s \in \S$}{
    \If{$\tau(x,s)=$\textit{sf}}{$\hat{d}_{x,s} = (\textit{atk,atk})$}
    \ElseIf{$\tau(x,s)=$\textit{c1}}{$\hat{d}_{x,s} = (\textit{rfc,atk})$}
    \ElseIf{$\tau(x,s)=$\textit{c2}}{$\hat{d}_{x,s} = (\textit{atk,rfc})$}
}

\Do{$t \leq T$}{$t \gets t+1$\;
    \For{every $s \in \S$}{
        \For{every $x \in \X$}{
            \If{$\tau(x,s)=$\textit{pf}}{
                Given $V^{(t)}$, Find deterministic joint single-axis strategy $\hat{d}_{x,s}$}
            }
        Create $\hat{\mathcal{A}}^1_s$ and $\hat{\mathcal{A}}^2_s$ from Alg. \ref{alg:getahat}\;
        $\hat{R}(\hat{V}^{(t-1)},s,a^1,a^2) \gets L(s) + \gamma  \sum_{s^\prime \in \S} P(s^\prime \ | \ s, a^{1},a^{2}) \cdot \hat{V}^{(t-1)}(s^\prime), \ \forall (a^1,a^2) \in \hat{\A}^1_s \times \hat{\A}^2_s$\;
        Follow procedure from Alg. \ref{alg:AVI}, lines 7-21, to find $\hat{V}^{(t)}(s)$    
        }
    }
    
\nl \KwRet{$\hat{V}^{(T)}$}
\end{algorithm}



%Furthermore, because CFH eliminates many dominated actions before $\hat{R}(s)$ is created, fewer lookups and less subsequent matrix reduction is required.

